Steric Engineering of Exciton Fine Structure in 2D Perovskites

A comprehensive study of excitonic properties of 2D layered perovskites is provided, with an emphasis on understanding and controlling the exciton fine structure. First, an overview of the optical properties is presented, discussing the challenges in determining the bandgap and exciton binding energies. Through magneto-optical spectroscopic measurements (up to B = 140 T), scaling laws are established for exciton binding energy as a function of the band gap and the diamagnetic coefficient. Using an in-plane magnetic field, the exciton fine structure for various 2D perovskites is examined to measure the energy splitting between the excitonic levels. The exciton fine structure and exchange interaction are correlated with structural parameters, employing an effective mass model, to highlight the role of steric effect on the exchange interaction. These findings reveal that lattice distortions, introduced by organic spacers, significantly influence the exchange interaction, driving a tunable energy spacing between dark and bright excitons. This unique feature of 2D perovskites, not present in other semiconductors, offers a novel tuning mechanism for exciton control, making these materials highly promising for efficient light emitters and advanced quantum technologies.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
